Formal Verification of an Out-of-Order Multiprocessor against an In-Order Weak-Memory ISA

Out-of-order multiprocessors are critical components of modern hardware, and their verification is desirable as they are difficult to correct once shipped. Existing literature simplifies and improves instruction set architectures (ISAs) for such processors, but they assume the processor correctly implements the ISA rather than proving it. We present the first formal verification of an out-of-order multiprocessor $\text{Core}_{\text{Impl}}$ against an in-order, weak-memory RISC-V ISA, RISC-V$_{\text{prom}}$. Our central component is $\text{Core}_{\text{InO}}$, an in-order one-instruction at a time core specification, enabling us to confine out-of-order reasoning to a single core. We decompose the main proof into two refinements. The core refinement proves that $\text{Core}_{\text{InO}}$ is a correct specification for $\text{Core}_{\text{Impl}}$. The system refinement shows that RISC-V$_{\text{prom}}$ is a correct specification for multiple $\text{Core}_{\text{InO}}$ connected with shared memory, leveraging the simplicity of $\text{Core}_{\text{InO}}$ in the proof. All of our proofs are mechanized in Rocq, with large language model agents heavily used to automate proof writing. We synthesized $\text{Core}_{\text{Impl}}$ into the Bluespec hardware description language, and validated it produces the intended weak behaviors and adheres to the official RISC-V test suite.

==> setup.tex <==
\makeatletter%
\@ifundefined{basedir}{%
\newcommand\basedir{}%
}{}%
\makeatother%

\makeatletter%

\providecommand*\@nameundef[1]{%
  \expandafter\let\csname #1\endcsname\@undefined}
\@nameundef{nequiv}
\@nameundef{state}

\makeatother%
\usepackage{url}
\usepackage{datetime}
\usepackage{xspace}
\usepackage{wasysym}
\usepackage{mathpartir}
\usepackage{dashbox}
\usepackage[inline]{enumitem}
\setlist{leftmargin=5.5mm,topsep=2mm}
\setlist[enumerate]{label=\textbf{(\arabic*)}}
\usepackage{colortbl}
\usepackage{tikz}
\usepackage{tcolorbox}
\usepackage{multirow}
\usepackage{hhline}
\usepackage{makecell}
\usepackage{booktabs}%
\newlist{tabitemize}{itemize}{1}
\setlist[tabitemize]{leftmargin=2.5mm,label=\textbullet,nosep,after=\strut}
\usepackage{tabularx}
\usepackage[inkscapearea=page]{svg}

\usepackage{algorithm}
\usepackage[rightComments=false,beginComment=//~,beginLComment=//~, endLComment=]{./algpseudocodex} %


\usepackage{pifont}

\usepackage{upquote}
\usepackage{kotex}
\usepackage{multicol}

\usepackage{wrapfig}
\usepackage{esvect}
\MakeRobust{\vv}

\usepackage{changepage}
\usepackage{amsmath}
\usepackage[export]{adjustbox}

\usepackage{siunitx}

\usepackage{\basedir pftools}
\usepackage{\basedir iris}


\usepackage{cleveref}

\usetikzlibrary{shapes}
\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{tikzmark}
\usetikzlibrary{fit}
\usetikzlibrary{shapes.multipart}
\usetikzlibrary{positioning}
\usetikzlibrary{chains}
\usetikzlibrary{backgrounds}
\tikzstyle{every picture}+=[remember picture]

\def\msf#1{\ensuremath{\mathsf{#1}}}

\newcommand{\isep}{\,\mathrel{*}\,}
\newcommand{\ISEP}{\mathop{\scalebox{4}{\raisebox{-0.2ex}{$\ast$}}\!}}
\newcommand{\ISep}[1]{%
  \ISEP
  \left\{\begin{array}{@{\,}l}
  #1
  \end{array}\right.
}

\newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{reqthm}{Requirement}
\newtheorem{stthm}{Observation}

\definecolor{StringRed}{rgb}{.637,0.082,0.082}
\definecolor{CommentGreen}{rgb}{0.0,0.55,0.3}
\definecolor{KeywordBlue}{rgb}{0.0,0.3,0.55}
\definecolor{HighlightColor}{rgb}{0.0,0.0,0.0}


\definecolor{grey}{rgb}{0.5,0.5,0.5}
\definecolor{red}{rgb}{1,0,0}
\definecolor{darkgreen}{rgb}{0.0,0.7,0.0}
\definecolor{lightpurple}{rgb}{1,0.7,.9}

\definecolor{circ-purple}{HTML}{D9D2E9}
\definecolor{circ-yellow}{HTML}{FFF2CC}
\definecolor{circ-green}{HTML}{D9EAD3}
\definecolor{hppp-pink}{HTML}{F4CCCC}

\crefname{section}{\textcolor{ACMPurple}{\S{}}}{\textcolor{ACMPurple}{\S{}}\!}
\crefformat{section}{\textcolor{ACMPurple}{#2\S{}#1#3}}
\Crefname{section}{Section}{Sections}
\Crefformat{section}{\textcolor{ACMPurple}{\S{}#2#1#3}}
\crefrangelabelformat{section}{\textcolor{ACMPurple}{#3#1#4}--\textcolor{ACMPurple}{#5#2#6}}

\Crefname{figure}{\textcolor{ACMPurple}{\text{Figure}}}{\textcolor{ACMPurple}{\text{Figures}}}
\crefname{figure}{\textcolor{ACMPurple}{\text{Fig.}}}{\textcolor{ACMPurple}{\text{Figs.}}}
\Crefname{table}{\textcolor{ACMPurple}{\text{Table}}}{\textcolor{ACMPurple}{\text{Tables}}}
\crefname{table}{\textcolor{ACMPurple}{\text{Table}}}{\textcolor{ACMPurple}{\text{Tables}}}

\crefname{algorithm}{\textcolor{ACMPurple}{\text{Algorithm} {}}}{\textcolor{ACMPurple}{\text{Algorithm} {}}\!}
\crefformat{algorithm}{\textcolor{ACMPurple}{#2\text{Algorithm} {}#1#3}}
\Crefname{algorithm}{\textcolor{ACMPurple}{\text{Algorithm}}}{\textcolor{ACMPurple}{\text{Algorithms}}}
\Crefformat{algorithm}{\textcolor{ACMPurple}{\text{Algorithm} {}#2#1#3}}
\crefrangelabelformat{algorithm}{\textcolor{ACMPurple}{#3#1#4--#5#2#6}}

\crefname{corollary}{\text{Corollary}}{\text{corollaries}}
\Crefname{corollary}{\text{Corollary}}{\text{Corollaries}}
\crefname{lemma}{\text{Lemma}}{\text{Lemmas}}
\Crefname{lemma}{\text{Lemma}}{\text{Lemmas}}
\crefname{theorem}{\text{Theorem}}{\text{Theorems}}
\Crefname{theorem}{\text{Theorem}}{\text{Theorems}}
\crefname{proposition}{\text{Prop.}}{\text{Propositions}}
\Crefname{proposition}{\text{Proposition}}{\text{Propositions}}
\crefname{definition}{\text{Def.}}{\text{Definitions}}
\Crefname{definition}{\text{Definition}}{\text{Definitions}}
\Crefname{reqthm}{\textcolor{ACMPurple}{\text{Requirement}}}{\textcolor{ACMPurple}{\text{Requirements}}}
\crefname{reqthm}{\textcolor{ACMPurple}{\text{Requirement}}}{\textcolor{ACMPurple}{\text{Requirements}}}
\Crefname{stthm}{\textcolor{ACMPurple}{\text{Observation}}}{\textcolor{ACMPurple}{\text{Observations}}}
\crefname{stthm}{\textcolor{ACMPurple}{\text{Observation}}}{\textcolor{ACMPurple}{\text{Observations}}}

\crefname{appendix}{\S{}}{\S{}\!}
\crefformat{appendix}{#2\S{}#1#3}
\Crefname{appendix}{Appendix}{Appendices}
\Crefformat{appendix}{\S{}#2#1#3}

\newcommand{\parhead}[1]{\noindentparagraph{\textbf{#1}.}}

\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\changed}[1]{\emph{\textcolor{KeywordBlue}{#1}}}
\newcommand{\circled}[1]{{\footnotesize {\Circled{#1}}}}

\newcommand{\aka}{a.k.a.\xspace}
\newcommand{\eg}{\emph{e.g.}\xspace}
\newcommand{\ie}{\emph{i.e.}\xspace}
\newcommand{\resp}{resp.\xspace}


\algrenewcommand\algorithmicindent{1.0em}
\newcommand*{\Continue}{\textbf{continue}}
\newcommand*{\Break}{\textbf{break}}

\makeatletter
\newcounter{algorithmicH}%
\let\oldalgorithmic\algorithmic
\renewcommand{\algorithmic}{%
  \stepcounter{algorithmicH}%
  \oldalgorithmic}%
\renewcommand{\theHALG@line}{ALG@line.\thealgorithmicH.\arabic{ALG@line}}
\makeatother

\AtBeginEnvironment{algorithmic}{%
  \sffamily
}

\algrenewcommand\textproc{}

\definecolor[named]{ACMPurple}{cmyk}{0.55,1,0,0.15}
\definecolor{StringRed}{rgb}{.637,0.082,0.082}
\definecolor{CommentGreen}{rgb}{0.0,0.55,0.3}
\definecolor{KeywordBlue}{rgb}{0.0,0.3,0.55}
\definecolor{LinkColor}{rgb}{0.55,0.0,0.3}
\definecolor{CiteColor}{rgb}{0.55,0.0,0.3}
\definecolor{hppp-cyan}{HTML}{D0E0E3}
\definecolor{hppp-purple}{HTML}{D9D2E9}
\definecolor{hppp-yellow}{HTML}{FFF2CC}
\definecolor{hppp-green}{HTML}{D9EAD3}
\definecolor{hppp-pink}{HTML}{F4CCCC}
\definecolor{hp-blue}{HTML}{D0E0E3}
\definecolor{shadecolor}{HTML}{FFF6F6}

\definecolor{grey}{rgb}{0.5,0.5,0.5}
\definecolor{red}{rgb}{1,0,0}
\definecolor{darkgreen}{rgb}{0.0,0.7,0.0}


\newcommand{\todotmpl}[3]{{\color{#2}[\textbf{#1}: {#3}]}}
\newcommand{\todo}[1]{{\raggedright\todotmpl{todo}{blue}{#1}\par}}
\newcommand*{\rfc}[1]{\todotmpl{RFC}{olive}{#1}}
\newcommand*{\jeehoon}[1]{\todotmpl{jeehoon}{purple}{#1}}
\newcommand*{\jungin}[1]{\todotmpl{jungin}{red}{#1}}
\newcommand*{\janggun}[1]{\todotmpl{janggun}{orange}{#1}}
\newcommand{\codex}[1]{{\raggedright\todotmpl{codex}{teal}{#1}\par}}
\newcommand*{\claude}[1]{\todotmpl{claude}{orange}{#1}}
\newcommand*{\claudesuggest}[1]{\todotmpl{claude suggest}{teal}{#1}}
\newcommand*{\jaehwang}[1]{\todotmpl{jaehwang}{darkgreen}{#1}}
\newcommand*{\jeonghyeon}[1]{\todotmpl{jeonghyeon}{CommentGreen}{#1}}
\newcommand*{\jeehooncomment}[1]{\todotmpl{jeehoon comment}{CommentGreen}{#1}}
\newcommand*{\discuss}[1]{\todotmpl{discuss}{olive}{#1}}


\newcommand*{\hpstand}{{Val\textsubscript{\textit{mark}}}\xspace}
\newcommand*{\hpimmut}{{Val\textsubscript{\textit{immut}}}\xspace}


\newcommand*{\revision}{\jeehoon{REVISED SO FAR}}


\DeclareMathOperator{\LSB}{LSB}
\DeclareMathOperator{\overapprox}{ceil}
\DeclareMathOperator{\maxepoch}{max}
\DeclareMathOperator{\expired}{expired}
\DeclareMathOperator{\transepoch}{trans}
\DeclareMathOperator{\untransepoch}{untrans}

\newcommand{\greenCheck}{\textcolor{CommentGreen}{\ding{51}}}%
\newcommand{\redX}{\textcolor{StringRed}{\ding{55}}}%
\newcommand{\yellowTriangle}{\textcolor{olive}{\ding{115}}}%

\usepackage{stmaryrd}

\definecolor{StringRed}{rgb}{.58,0.06,0.06}
\definecolor{CommentGreen}{rgb}{0.0,0.55,0.3}
\definecolor{KeywordBlue}{rgb}{0.0,0.3,0.55}
\definecolor{LinkColor}{rgb}{0.55,0.0,0.3}
\definecolor{CiteColor}{rgb}{0.55,0.0,0.3}
\definecolor{HighlightColor}{rgb}{0.0,0.0,0.0}
\definecolor{Protected}{rgb}{.20,.50,.70} %
\definecolor{Managed}{rgb}{.64,.40,.20} %
\definecolor{ProofShade}{cmyk}{0,0,0,0.05}

\newcommand{\ghostVar}[3]{\ownGhost{}{#1 \Mapsto^{#2} #3}}
\newcommand{\natauth}[2]{\ownGhost{#1}{\authfull \textlog{MN}\ #2}}
\newcommand{\natfrag}[2]{\ownGhost{#1}{\authfrag \textlog{MN}\ #2}}
\newcommand{\mapauth}[2]{\ownGhost{#1}{\authfull \textlog{Map}\ #2}}
\newcommand{\mapfrag}[3]{\ownGhost{#1}{\authfrag \textlog{Map}\ #2 \mapsto ^{\always} #3}}
\newcommand{\mapfraghalf}[3]{\ownGhost{#1}{\authfrag \textlog{Map}\ #2 \mapsto ^{1/2} #3}}

\newcommand*\Ndom{\namesp_\textrm{dom}}
\newcommand*\Nptr{\namesp_\textrm{ptr}}
\newcommand*\Domain{\msf{Domain}}
\newcommand*\NodeRes{\textdom{NodeRes}}
\newcommand*\Managed{\msf{Managed}}
\newcommand*\Shield{\msf{HPSlot}}
\newcommand*\Protected{\msf{Protected}}
\newcommand*\Guard{\msf{RCUSlot}}
\newcommand*\pGuard{\msf{\color{Protected}Guard}}
\newcommand*\Deactivated{\msf{Deactivated}}
\newcommand*\Unprotected{\msf{Unprotected}}
\newcommand*\Activated{\msf{\color{Protected}Activated}}
\newcommand*\NotValidated{\msf{NotValidated}}
\newcommand*\Validated{\msf{\color{Protected}Validated}}
\newcommand*\RCUState{\msf{RCUState}}
\newcommand*\RCUNodeInfo{\msf{RCUNodeInfo}}
\newcommand*\RCUPointsTo{\msf{RCUPointsTo}}
\newcommand*\Deleted{\msf{Deleted}}

\newcommand*\ThreadId{\textdom{ThreadId}}
\newcommand*\NodeId{\textdom{NodeId}}
\newcommand*\Resource{\msf{Resource}}
\newcommand*\ResourceTok{\msf{ResourceTok}}
\newcommand*\Exchanges{\msf{Exchanges}}

\newcommand{\find}{\code{find}}
\newcommand{\prev}{\code{prev}}
\newcommand{\curr}{\code{curr}}
\newcommand{\clist}{\code{hl}}
\newcommand{\prevnext}{\code{prev\_next}}
\newcommand{\cvalue}{\code{value}}
\newcommand{\true}{\code{true}}
\newcommand{\false}{\code{false}}
\newcommand{\NONE}{\code{None}}
\newcommand{\SOME}{\code{Some}}

\newcommand{\LIST}{\msf{List}}
\newcommand{\Map}{\msf{Map}}
\newcommand{\Set}{\msf{Set}}
\newcommand{\HSet}{\msf{HSet}}
\newcommand{\IsHSet}{\msf{IsHSet}}
\newcommand{\HList}{\msf{HList}}
\newcommand{\IsHList}{\msf{IsHList}}
\newcommand{\HListInv}{\msf{HListInv}}
\newcommand{\gnlist}{\gname_{\clist}}
\newcommand{\gnl}{\gname_{l}}
\newcommand{\gnp}{\gname_{p}}
\newcommand{\listapp}{\code{++}}
\newcommand{\app}{\mathbin{+\!\!+}}
\newcommand{\Sorted}{\msf{Sorted}}
\newcommand{\ANodes}{\msf{ANodes}}
\newcommand{\CNodes}{\msf{CNodes}}
\newcommand{\Node}{\msf{Node}}
\newcommand{\data}{\msf{data}}
\newcommand{\loc}{\msf{loc}}
\newcommand{\marked}{\msf{marked}}
\newcommand{\Proph}{\msf{Proph}}
\newcommand{\MChain}{\msf{MChain}}
\newcommand{\GhostMap}{\msf{GMap}}

\newcommand{\Rob}{\msf{ROB}}
\newcommand{\Rf}{\msf{RF}}
\newcommand{\Alu}{\msf{ALU}}
\newcommand{\Mem}{\msf{MemUnit}}
\newcommand{\Lsq}{\msf{LSQ}}
\newcommand{\Stb}{\msf{StB}}
\newcommand{\Rs}{\msf{RS}}
\newcommand{\SMan}{\msf{SMan}}
\newcommand{\StsBag}{\msf{StsBag}}
\newcommand{\LdsBag}{\msf{LdsBag}}
\newcommand{\SIListT}{\msf{SIList}}
\newcommand{\ShMem}{\msf{ShMem}}
\newcommand{\DMem}{\msf{DMem}}
\newcommand{\IMem}{\msf{IMem}}
\newcommand{\ISA}{\msf{ISA}}
\newcommand{\ISACF}{\ensuremath{\msf{ISA}_{CF}}}
\newcommand{\CoreI}{\ensuremath{\msf{Core}_{Impl}}}
\newcommand{\CoreL}{\ensuremath{\msf{Core}_{\msf{Impl}}}}
\newcommand{\CoreS}{\ensuremath{\msf{Core}_s}}
\newcommand{\CoreSF}{\ensuremath{\msf{Core}_{\msf{MemFin}}}}
\newcommand{\CoreIO}{\ensuremath{\msf{Core}_{\msf{InO}}}}
\newcommand{\CoreOoO}{\ensuremath{\msf{Core}_{\msf{OoO}}}}
\newcommand{\TopMod}{\msf{TopMod}}
\newcommand{\RISCVPROM}{\ensuremath{\msf{RISC\text{-}V}_{\msf{prom}}}}
\newcommand{\RISCV}{\ensuremath{\msf{RISC\text{-}V}}}
\newcommand{\TId}{\msf{CId}}
\newcommand{\ValT}{\msf{Val}}
\newcommand{\AddrT}{\msf{Addr}}


